Swarm intelligence for full Stokes dynamic imaging reconstruction of interferometric data

In very long baseline interferometry (VLBI) the combination of multiple antennas permits the synthesis of a virtual telescope with a larger diameter and consequently higher resolution than the individual antennae. Yet, due to the sparse nature of the array, recovering an image from the observed data is a challenging ill-posed inverse problem. The VLBI community is interested in not only recovering an image in total intensity from interferometric data, but also to obtain results in the polarimetric and the temporal domain. Only a few algorithms are able to work in all these domains simultaneously. In particular, the algorithms based on optimization that consider various penalty terms specific to static total intensity imaging, time-variability and polarimetry are restricted to grids the domain of the objective function. In this work we present a novel algorithm, multiobjective particle swarm optimization, that is able to recover the optimal weights without any space-gridding, and to obtain the marginal contribution of each the playing terms. To this end, we utilize multiobjective optimization together with particle swarm metaheuristics. We let the swarm of weights to converge together to the best position. We evaluate our algorithm with representative synthetic data sets focused on the instrumental configuration of the Event Horizon Telescope Collaboration and its planned successors. We successfully recover the polarimetric, static and time-dynamic signature of the ground truth movie, even with relative sparsity, and a set of realistic data corruptions. This is a novel, fast, weighting space gridding-free algorithm that successfully recovers static and dynamic polarimetric reconstructions. Compared to Regularized Maximum Likelihood methods, it avoids the need for parameter surveys, and it is not limited to the number of pixels such as recently proposed multiobjective imaging algorithms.

==> appendices.tex <==
\section{Polarimetry} \label{app: polarimetry}


To demonstrate the capabilities of PSO imaging in the polarimetric domain, we replicate the experiments presented in \citet{Mueller2022c} and~\cite{Mus2023b}, using a synthetic data source out of the \textit{ehtim} software package \citep{Chael2016, Chael2018}. 

For the polarimetric reconstruction, we follow a similar strategy than for~\citetalias{Mus2023b} we fixed the Stokes I reconstruction, and only solved for linear polarization. We initialized the initial population with images with constant electric vector position angle (EVPA) at a constant polarization fraction of $1\%$ across the whole field of view. Rather than with the Stokes parameters $Q, U$, we equivalently model the linear polarization by the linear polarization fraction $m$ and the mixing angle $\chi$, i.e.:
\begin{align}
    Q + iU = m \cdot I \cdot e^{2\pi i \chi}.
\end{align}
This turns out to be beneficial since inequality \eqref{eq: stokes_inequality} is automatically satisfied by imposing $0 \leq m \leq 1$, specifically we cannot create spurious polarimetric signals outside of the total intensity contours.

To verify that PSO reconstructions performs well for a wider range of EVPA structures on such a challenging data set as the EHT observations, we performed a number of additional tests with an artificial ring image and different EVPA patterns (toroidal magnetic field, radial magnetic field and a vertical magnetic). Fig.~\ref{fig: rings1}, Fig. \ref{fig: rings2} and Fig. \ref{fig: rings3} show the true model (left panel) and recover PSO image (right panel). The reconstruction of the overall pattern is successful in all four cases. In conclusion, we can differentiate various magnetic field configurations by the PSO reconstructions of EHT like data.

\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{Figures/model1.pdf}
    \caption{Simulated ring-like source with vertical EVPA using EHT 2017 array. Left panel: Ground truth. Right panel: pso ireconstrucion (solution). The top panel show the reconstructions at full resolution, the bottom panels blurred with a resolution of $20\,\mu\mathrm{as}$. Vertical lines represent the EVPA and their color, the amount of polarization fraction. The color map for the brightness of the source is different to the one of the EVPAs.}
    \label{fig: rings1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{Figures/model2.pdf}
    \caption{Same as Fig. \ref{fig: rings2}, but for a toroidal magnetic field.}
    \label{fig: rings2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[scale=0.5]{Figures/model3.pdf}
    \caption{Same as Fig. \ref{fig: rings2}, but for a toroidal magnetic field.}
    \label{fig: rings3}
\end{figure*}

\section{Recovered Movie at MOEA/D resolution} \label{app: coarse}
We show the recovered movie with MO-PSO in Fig. \ref{fig: reco_movie}. The same observation data have been recovered already in \citet{Mus2023b} with MOEA/D, although with a smaller resolution due to the limitations with respect to numerical performance. To simplify comparisons we present in Fig. \ref{fig: reco_movie_coarse} the recovered movie with MO-PSO, but regridded to the same resolution and field of view as presented in \citetalias{Mus2023b}.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{Figures/reco_movie_coarse.png}
    \caption{Same as Fig. \ref{fig: reco_movie}, but regridded to the field of view $180\mu\mathrm{as}$ and resolution $10\mu\mathrm{as}$ as was used in \citetalias{Mus2023b}.}
    \label{fig: reco_movie_coarse}
\end{figure*}

% \subsection{Dynamics}

% We test the algorithm using two datasets with different uv-coverages and we compare solutions with the obtanied using the MOEA/D.
% The first data set, a more simple one, is based on the one presented in~\cite{Johnson2017, shiokawa2013}, and the data was shared by private communication \textbf{I WOULD FEEL MORE COMFY IF WE DROP HIM AN EMAIL ASKING PERMISSION}. This data only contains Stokes I information. We call this data \texttt{MJ2017}.
% The second synthetic data, called \texttt{CH3} set is the one given for the \texttt{Challlenge 3} presented in~\cite{ngehtchallenge}\footnote{\url{https://challenge.ngeht.org/}}. The synthetic data of this last dataset is dynamically polarized, i.e., the intrinsic polarization structe of the source varies along the observation. Therefore, we show an example of a joint polarimetric and dynamic reconstruction, and thus we will see how MOEA/D solves for polarimetric movies and dynamics are not limited to Stokes I 

% \subsection{\texttt{MJ2017} data}

% To assess the performance of MOEA/D in dynamic reconstruction, we replicated the experiment conducted by~\cite{Johnson2017} for verification purposes. Specifically, we reconstructed the keyframes presented in Figure 4 of their work, which correspond to time instances at 16:00 UTC, 00:43:26 UTC and 06:29:27 UTC. These keyframes represent subsets of antennas observed within the EHT 2017 array configuration. The first keyframe involves 4 antennas, the second 5 antennas, and the final one only 2 antennas. The differing numbers of baselines between these keyframes render the reconstruction of a continuous movie through snapshot imaging unfeasible. A comprehensive comparison between the performance of ngMEM and the regularizers proposed by~\cite{Johnson2017} in this specific scenario is detailed in~\cite{Mus2023}.\\
% \\
% To generate a comparable movie, our approach initially constructing a static image utilizing 24 hours of observation data. Subsequently, we flagged all visibilities corresponding to the aforementioned timestamps. Employing the static image as an initial reference point within our algorithm, we executed MOEA/D to facilitate the reconstruction process.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/mj_movie.pdf}
%     \caption{PSO movie reconstruction for }
%     \label{fig:mj_reconstruction_case}
% \end{figure*}
